Causal Dynamics of Discrete Surfaces

We formalize the intuitive idea of a labelled discrete surface which evolves in time, subject to two natural constraints: the evolution does not propagate information too fast; and it acts everywhere the same.

==> eptcsdata.tex <==
\providecommand{\firstpage}{30}
\providecommand{\publicationstatus}{M. Ayala-Rinc\'on E. Bonelli and I. Mackie (Eds): \\ Developments in Computational Models (DCM 2013)\\
EPTCS 144, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.144.3}{10.4204/EPTCS.144.3}}
\pdfoutput=1

